NetKernel: Making Network Stack Part of the Virtualized Infrastructure

This paper presents a system called NetKernel that decouples the network stack from the guest virtual machine and offers it as an independent module. NetKernel represents a new paradigm where network stack can be managed as part of the virtualized infrastructure. It provides important efficiency benefits: By gaining control and visibility of the network stack, operator can perform network management more directly and flexibly, such as multiplexing VMs running different applications to the same network stack module to save CPU cores, and enforcing fair bandwidth sharing with distributed congestion control. Users also benefit from the simplified stack deployment and better performance. For example mTCP can be deployed without API change to support nginx natively, and shared memory networking can be readily enabled to improve performance of colocated VMs. Testbed evaluation using 100G NICs shows that NetKernel preserves the performance and scalability of both kernel and userspace network stacks, and provides the same isolation as the current architecture.

==> Makefile <==
# Makefile for LaTeX document files
# Created by Baochun Li, bli@eecg.toronto.edu, March 30 2001
# Last modified: September 27 2002 

DOCUMENT=main

default: $(DOCUMENT).pdf

$(DOCUMENT).toc: $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

$(DOCUMENT).pdf: $(DOCUMENT).toc
	bibtex $(DOCUMENT)
	pdflatex $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

#--------------------------------------------------
# $(DOCUMENT).ps: $(DOCUMENT).dvi
# 	dvips -t letter -Ppdf -G0 -o $@ $<
# 
# $(DOCUMENT).pdf: $(DOCUMENT).ps
# 	cat $(DOCUMENT).ps | ps2pdf - > $(DOCUMENT).pdf 
#-------------------------------------------------- 

all: $(DOCUMENT).pdf

clean:
	rm -rf *.aux $(DOCUMENT).log $(DOCUMENT).toc \
     $(DOCUMENT).bbl $(DOCUMENT).blg *.bak \
		 $(DOCUMENT).out *.log *.gz\
      $(DOCUMENT).pdf *.fls 

open:
	open $(DOCUMENT).pdf

gopen:
	gnome-open $(DOCUMENT).pdf

opens:
	open $(DOCUMENT).tex

gopens:
	gnome-open $(DOCUMENT).tex



==> future.tex <==
%!TEX root = main.tex

\section{Future work}
\label{sec:future_work}
We plan to extend this different aspects. First, we will implement NetKernel in linux kernel to improve the efficiency. Second, more NSM images will be fostered, including different transport-protocols (e.g. DCTCP, RDMA), OS optimizations, and network functions. Finally, we will experiment NetKernel in more complex environments.

